An end-to-end data-driven optimisation framework for constrained trajectories

Many real-world problems require to optimise trajectories under constraints. Classical approaches are based on optimal control methods but require an exact knowledge of the underlying dynamics, which could be challenging or even out of reach. In this paper, we leverage data-driven approaches to design a new end-to-end framework which is dynamics-free for optimised and realistic trajectories. We first decompose the trajectories on function basis, trading the initial infinite dimension problem on a multivariate functional space for a parameter optimisation problem. A maximum \emph{a posteriori} approach which incorporates information from data is used to obtain a new optimisation problem which is regularised. The penalised term focuses the search on a region centered on data and includes estimated linear constraints in the problem. We apply our data-driven approach to two settings in aeronautics and sailing routes optimisation, yielding commanding results. The developed approach has been implemented in the Python library PyRotor.

==> adjustment.tex <==
\subsection{Aerodynamic constraints verification through an iterative procedure}

blabla


\subsection{Handling reference trajectories with different durations}

In the setting of Section \ref{sec:opti}, the reference trajectories are implicitly assumed to have the same duration $T$ but this may not be the case in practice. For instance, if one is interested in optimising the climb phase for aircraft from a given altitude to a final one, then one may observe duration differences which vary from a few seconds to a few minutes. In such a case, projecting these trajectories onto the same functional basis is not possible and the approach developed in Section \ref{sec:opti} can not be applied.

To deal with this problem, we propose to extend each reference trajectory $y_{R_i} \in L^2\big([0,T_i], \R^D \big)$ to a trajectory $\overline{y}_{R_i}$ over a larger time interval $[0, T]$ defined as follows:
\begin{equation*}
    \overline{y}_{R_i}(t) := \left\{
    \begin{array}{l}
        y_{R_i}(t) \; , \quad \text{if } t \in [0, T_i] \\[2mm]
        y_{fin} \; , \quad \text{if } t \in [T_i, T]
    \end{array} \right. \; ,
\end{equation*}
where we set $\displaystyle T := \max_{i \in \{1, \dots, I\}} T_i$. In the climb optimisation setting, this consists in concatenating the beginning of an artificial cruise to each reference climb. Thanks to this procedure, it is then possible to project each component of the reference flights on an orthonormal basis of $L^2\big([0,T], \R \big)$. In this setting, we consider then the following optimisation problem:
\begin{equation*}
    \overline{y}^\star \in \argmin_{y \in \mathcal{Y}_\mathcal{K}(0,T) \cap \mathcal{B}(y_{init}, y_{fin})} \sum_{i=1}^I \omega_i \int_0^T \Big\| \Lambda^{\frac{1}{2}} \big( y(t) - \overline{y}_{R_i}(t) \big) \Big\|_{\R^D}^2 \, dt + \int_0^T \FF\big(y(t) \big) \, dt \; ,
\end{equation*}
which is equivalent of an optimisation problem on $\R^K$ of the form \eqref{eq:opt_c2} according to \autoref{prop:min_pb_equiv_y_C}.

On the other hand, the duration $T$ to reach the final state $y_{fin}$ from the initial one $y_{init}$ following the trajectory $\overline{y}^\star$ may be too large when compared to the durations $T_i$ of the best reference trajectories. Nevertheless the trajectory $\overline{y}^\star$ may be close to (even reach) the final state $y_{fin}$ before the final time $T$; for instance, this is likely to occur if the duration of the reference trajectories associated with the largest weights are smaller than $T$. We exploit this fact to propose a truncation-adjustment step leading to an optimised trajectory with a more realistic duration in this setting while remaining close to the optimised trajectory $\overline{y}^\star$. We proceed as follows:
\begin{enumerate}
    \item \underline{Truncation:}\\
    Suppose that the set
    \begin{equation*}
        \Big\{t \in [0,T] \, \Big| \, \Big\| \Lambda^{\frac{1}{2}} \big( \overline{y}^\star(t) - y_{fin} \big) \Big\|_{\R^D}^2 \leqslant \epsilon \Big\} \; ,
    \end{equation*}
    where $\epsilon > 0$, is non-empty and take its minimal element $T_\epsilon$ (or infimum). If the error $\epsilon$ is acceptable from an expert point of view, then the truncated trajectory $\overline{y}^\star|_{[0,T_\epsilon]}$ is the output of our optimisation process. Otherwise we consider the two following steps to adjust $\overline{y}^\star|_{[0,T_\epsilon]}$ so that the resulting trajectory satisfies the endpoint constraints.
    \item \underline{Projection:}\\
    We set $y_\epsilon := \overline{y}^\star|_{[0,T_\epsilon]}$. The truncated trajectory $y_\epsilon$ does not belong necessarily to a finite dimension space. Given $\varepsilon > 0$, we choose $\mathcal{K}_\varepsilon = \big\{K_{\varepsilon,1},\dots,K_{\varepsilon,D} \big\}$ such that the projection $\widetilde{y}_\epsilon$ of $y_\epsilon$ onto $\mathcal{Y}_{\mathcal{K}_\varepsilon}(0,T_\epsilon)$ satisfies 
    \begin{equation*}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( \widetilde{y}_\epsilon(t) - y_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \leqslant \varepsilon \; .
    \end{equation*}
    We define
    \begin{equation*}
        c_\epsilon := \Phi \, y_\epsilon \in \R^{K_\varepsilon} \qquad , \qquad \widetilde{y}_\epsilon := \Phi|_{\mathcal{Y}_\epsilon(0,T_\epsilon)}^{-1} c_\epsilon \in \mathcal{Y}_{\mathcal{K}_\varepsilon}(0,T_\epsilon) \; ,
    \end{equation*}
    where $K_\varepsilon := \sum_{d=1}^D (1 + K_{\varepsilon,d})$. Note that the projected trajectory $\widetilde{y}_\epsilon$ is likely not to satisfy the endpoint constraints, \emph{i.e.} $\widetilde{y}_\epsilon \notin \mathcal{B}(y_{init}, y_{fin})$.
    \item \underline{Penalised adjustment:}\\
    To obtain a final trajectory belonging to $\mathcal{B}(y_{init}, y_{fin})$, we slightly modify the projected trajectory $\widetilde{y}_\epsilon$ so that the endpoint constraints are verified. To do so, we propose to solve the following optimisation problem:
    \begin{equation} \label{eq:pen_adj}
        y_\eta^\star \in \argmin_{y \in \mathcal{Y}_{\mathcal{K}_\varepsilon}(0,T_\epsilon) \cap \mathcal{B}(y_{init}, y_{fin})} \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt + \eta \int_0^{T_\epsilon} \FF\big(y(t) \big) \, dt \; ,
    \end{equation}
    where $\eta > 0$, which is equivalent to the following one according to \autoref{prop:min_pb_equiv_y_C}:
    \begin{equation} \label{eq:pend_adj_c} 
        c_\eta^\star \in \argmin_{c \in \mathcal{C}(y_{init}, y_{fin})} \Big\| \overline{\Lambda}^{\frac{1}{2}} \big(c - c_\epsilon \big) \Big\|_{\R^K_\varepsilon}^2 + \eta \, \TFC(\Phi|_{\mathcal{Y}_\epsilon(0,T_\epsilon)}^{-1} c) \; .
    \end{equation}
    Here we choose $\eta > 0$ sufficiently small so that the preceding optimisation problem is strictly convex, namely the cost function is strictly convex.
\end{enumerate}

In the following theorem, we show that the total fuel consumption of $y_\eta^\star$ is necessarily smaller than the one of $\widetilde{y}_\epsilon$. Further we prove that the trajectories $y_\eta^\star$ and $y_\epsilon$ are close if $\eta$ is sufficiently small, if the projected trajectory $\widetilde{y}_\epsilon$ is sufficiently accurate and if the endpoint constraints errors of $\widetilde{y}_\epsilon$ are sufficiently small.
\begin{theorem} \label{thm:stablity_adj}
    The solution $y_\eta^\star$ of the optimisation problem \eqref{eq:pen_adj} satisfies the following property:
    \begin{equation} \label{eq:TFC_adjust}
        \TFC(y_\eta^\star) \leqslant \TFC(\widetilde{y}_\epsilon) - \eta^{-1} \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_\eta^\star(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \; .
    \end{equation}
    Assume in addition the matrix $A(0,T_\epsilon) \in \R^{2D \times K_\varepsilon}$ defined in \autoref{prop:linear_const} to be full rank and that there exists $\delta > 0$ such that
    \begin{equation*}
        \Big\| \Lambda^\frac{1}{2} \big (\widetilde{y}_\epsilon(0) - y_{init} \big) \Big\|_{\R^D}^2 + \Big\| \Lambda^\frac{1}{2} \big (\widetilde{y}_\epsilon(T_\epsilon) - y_{fin} \big) \Big\|_{\R^D}^2 \leqslant \delta \; .
    \end{equation*}
    Let $\varepsilon > 0$. Then there exists $\eta_\varepsilon > 0$ such that for all $\eta \in (0, \eta_\varepsilon)$ we have
    \begin{equation} \label{eq:traj_adjust}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_\eta^\star(t) - y_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \leqslant 4 (\lambda_{max} + 1) \, \varepsilon +  \frac{4 \kappa}{\sigma_{min}^2} \, \delta \; ,
    \end{equation}
    where $\sigma_{min} > 0$ is the smallest singular value of the matrix $A(0,T_\epsilon)$ and
    \begin{equation*}
        \lambda_{max} := \max_{d \in \{1,\dots, D\}} \lambda^{(d)} \qquad , \qquad \kappa := \frac{\max_{d \in \{1,\dots, D\}} \lambda^{(d)}}{\min_{d \in \{1,\dots, D\}} \lambda^{(d)}} \; .
    \end{equation*}
\end{theorem}
\begin{proof}
    The trajectory $y_\eta^\star$ is the solution of the minimisation problem \eqref{eq:pen_adj}. Since $\widetilde{y}_\epsilon$ belongs also to $\mathcal{Y}_{\mathcal{K}_\varepsilon}(0,T_\epsilon) \cap \mathcal{B}(y_{init},y_{fin})$, we have
    \begin{align*}
        & \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_\eta^\star(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt + \eta \int_0^{T_\epsilon} \FF\big(y_\eta^\star(t) \big) \, dt \\
        & \hspace{2cm} \leqslant \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( \widetilde{y}_\epsilon(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt + \eta \int_0^{T_\epsilon} \FF\big(\widetilde{y}_\epsilon(t) \big) \, dt \\
        & \hspace{2cm} = \eta \int_0^{T_\epsilon} \FF\big(\widetilde{y}_\epsilon(t) \big) \, dt \; ,
    \end{align*}
    which leads to inequality \eqref{eq:TFC_adjust}.\\
    We prove now the second inequality \eqref{eq:traj_adjust}. First of all, we apply \autoref{lem:continuity_pert} whose hypotheses are satisfied with
    \begin{itemize}
        \item $A = A(0,T_\epsilon) \in \R^{2D \times K_\varepsilon}$ which is surjective by hypothesis;
        \item $b = (y_{init}, y_{fin})^T$;
        \item $\displaystyle f(c) = \Big\| \overline{\Lambda}^\frac{1}{2} (c - c_\epsilon) \Big\|_{\R^{K_\varepsilon}}^2$ which is a strictly convex $\mathcal{C}^\infty$-function;
        \item $g(c) = \TFC\big( \Phi|_{\mathcal{Y}_\epsilon(0,T_\epsilon)}^{-1} c \big)$ which is a $\mathcal{C}^\infty$-function.
    \end{itemize}
    This implies the continuity at 0 of the solution $c_\eta^\star$ of the optimisation problem \eqref{eq:pend_adj_c} with respect to $\eta$. Hence there exists $\eta_\varepsilon > 0$ such that
    \begin{equation*}
        \forall \, \eta \in (0, \eta_\varepsilon) \qquad \big\| c_\eta^\star - c_0^\star \big\|_{\R^{K_\varepsilon}}^2 \leqslant \varepsilon \; .
    \end{equation*}
    By \autoref{prop:phi_unitary}, it follows
    \begin{equation} \label{eq:ineq_1}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_\eta^\star(t) - y_0^\star(t) \big) \Big\|_{\R^D}^2 \, dt = \Big\| \overline{\Lambda}^\frac{1}{2} \big( c_\eta^\star - c_0^\star \big) \Big\|_{\R^{K_\varepsilon}}^2 \leqslant \lambda_{max} \, \varepsilon \; ,
    \end{equation}
    for all $\eta \in (0, \eta_\varepsilon)$. Furthermore the hypotheses of \autoref{lem:stability_adj} are satisfied so we have
    \begin{equation} \label{eq:ineq_2}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_0^\star(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \leqslant \frac{\kappa(\Lambda)}{\sigma_0\big(A(0,T_\epsilon)\big)^2} \, \delta \; .
    \end{equation}
    And the set $\mathcal{K}_\varepsilon$ is chosen in such way that
    \begin{equation} \label{eq:ineq_3}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( \widetilde{y}_\epsilon(t) - y_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \leqslant \varepsilon \; .
    \end{equation}
    By the parallelogram law, one has
    \begin{align*}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_\eta^\star(t) - y_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt
        & \leqslant 4 \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_\eta^\star(t) - y_0^\star(t) \big) \Big\|_{\R^D}^2 \, dt \\
        & \hspace{1cm} + 4 \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_0^\star(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \\
        & \hspace{2cm} + 4 \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( \widetilde{y}_\epsilon(t) - y_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \; .
    \end{align*}
    Inserting inequalities \eqref{eq:ineq_1}, \eqref{eq:ineq_2} and \eqref{eq:ineq_3} into the preceding one leads to the final result.
\end{proof}

\begin{lemma} \label{lem:stability_adj}
    Assume that there exist $\delta > 0$ such that
    \begin{equation*}
        \Big\| \Lambda^\frac{1}{2} \big (\widetilde{y}_\epsilon(0) - y_{init} \big) \Big\|_{\R^D}^2 + \Big\| \Lambda^\frac{1}{2} \big (\widetilde{y}_\epsilon(T_\epsilon) - y_{fin} \big) \Big\|_{\R^D}^2 \leqslant \delta \; ,
    \end{equation*}
    and assume that the matrix $A(0,T_\epsilon) \in R^{2D \times K_\varepsilon}$ is full rank. Then the solution of the optimisation problem
    \begin{equation} \label{eq:adj}
        y_0^\star \in \argmin_{y \in \mathcal{Y}_{\mathcal{K}_\varepsilon}(0,T_\epsilon) \cap \mathcal{B}(y_{init}, y_{fin})} \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt
    \end{equation}
    satisfies
    \begin{equation*}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_0^\star(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt \leqslant \frac{\kappa}{\sigma_{min}^2} \, \delta \; ,
    \end{equation*}
    where $\kappa$ and $\sigma_{min}$ are defined in \autoref{thm:stablity_adj}.
\end{lemma}
\begin{proof}
    First of all, we consider the following minimisation problem
    \begin{equation*}
        c_0^\star \in \argmin_{c \in \mathcal{C}(y_{init}, y_{fin})} \Big\| \overline{\Lambda}^{\frac{1}{2}} \big(c - c_\epsilon \big) \Big\|_{\R^{K_\varepsilon}}^2 \; ,
    \end{equation*}
    which is equivalent to the problem \eqref{eq:adj} following the lines of the proof of \autoref{prop:min_pb_equiv_y_C}.\\
    Consider now the singular value decomposition of the matrix $A(0,T_\epsilon)$:
    \begin{equation*}
        A(0,T_\epsilon) = U \Sigma V^T \; ,
    \end{equation*}
    where $\Sigma \in \R^{2D \times K_\varepsilon}$ is a rectangular diagonal matrix and $U \in \R^{2D \times 2D}$ and $V \in \R^{K_\varepsilon \times K_\varepsilon}$ are orthogonal matrices. In particular we can write
    \begin{equation*}
        U \Sigma V^T = U \Big( \Sigma_1 \hspace{3mm} 0_{2D, K_\varepsilon-2D} \Big) \left(
        \begin{array}{c}
            V_1^T \\[2mm]
            V_2^T
        \end{array} \right) = U \Sigma_1 V_1^T \; ,
    \end{equation*}
    where $\Sigma_1 \in \R^{2D \times 2D}$ is a diagonal matrix whose diagonal elements $\{ \sigma_d \}_{d=1}^{2D}$ are the singular values in descending order and $V_1 \in \R^{K_\varepsilon \times 2D}$ is a semi-orthogonal matrix; note that $\Sigma_1$ is non-singular and that $\sigma_d > 0$ for all $d \in \{1,\dots,2D\}$ thanks to the hypothesis $A(0,T_\epsilon)$ is full rank.\\
    For all $c \in \mathcal{C}(y_{init}, y_{fin})$, we have the following equivalences:
    \begin{align}
        A(0,T_\epsilon) c = \left(
        \begin{array}{c}
             y_{init} \\
             y_{fin} 
        \end{array} \right) \quad
        & \Longleftrightarrow \quad U \Sigma_1 V_1^T c = \left(
        \begin{array}{c}
             y_{init} \\
             y_{fin} 
        \end{array} \right) \nonumber \\
        & \Longleftrightarrow \quad V_1^T c = \Sigma_1^{-1} U^T \left(
        \begin{array}{c}
             y_{init} \\
             y_{fin} 
        \end{array} \right) \; . \label{eq:equiv_end_const}
    \end{align}
    Let now define the following vector $\widetilde{c} \in \R^{K_\varepsilon}$ through its image $V^T \widetilde{c}$:
    \begin{equation*}
        \left\{ \begin{array}{l}
            V_1^T \widetilde{c} = \Sigma_1^{-1} U^T \left(
        \begin{array}{c}
             y_{init} \\
             y_{fin} 
        \end{array} \right) \\[4mm]
        V_2^T \widetilde{c} = V_2^T c_\epsilon   
        \end{array} \right. \; .
    \end{equation*}
    We deduce that $\widetilde{c}$ belongs to $\mathcal{C}(y_{init},y_{fin})$ from the equivalences \eqref{eq:equiv_end_const} and we have
    \begin{align}
        \Big\| A(0,T_\epsilon) (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2
        & = \Big\| U \Sigma V^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2 \nonumber \\
        & = \Big\| \Sigma_1 V_1^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2 \label{eq:U_unit} \\
        & = \sum_{d = 1}^{2D} \sigma_d^2 \Big| \big(V_1^T \widetilde{c}\big)_d - \big(V_1^T c_\epsilon\big)_d \Big|^2 \nonumber \\
        & \geqslant \sigma_{2D}^2 \Big\| V_1^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2 \label{eq:min_sing_val} \\
        & = \sigma_{2D}^2 \Big\| V^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{K_\varepsilon}}^2 \label{eq:V_2_zero} \\
        & = \sigma_{2D}^2 \big\| \widetilde{c} - c_\epsilon \big\|_{\R^{K_\varepsilon}}^2 \label{eq:V_unit} \; ;
    \end{align}
    \begin{itemize}
        \item \eqref{eq:U_unit}: use the unitary property of $U$ and the equality $U \Sigma V^T = U \Sigma_1 V_1^T$;
        \item \eqref{eq:min_sing_val}: use the fact that $\sigma_d \geqslant \sigma_{2D}$ for all $d \in \{1, \dots, 2D \}$;
        \item \eqref{eq:V_2_zero}: by the definition of $\widetilde{c}$, we have
        \begin{equation*}
            \Big\| V^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{K_\varepsilon}}^2 = \Big\| V_1^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2 + \Big\| V_2^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{K_\varepsilon-2D}}^2 = \Big\| V_1^T (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2 \; ;
        \end{equation*}
        \item[\eqref{eq:V_unit}]: use the unitary property of $V$.
    \end{itemize}
    It follows
    \begin{align}
        & \Big\| \overline{\Lambda}^\frac{1}{2} (\widetilde{c} - c_\epsilon ) \Big\|_{\R^{K_\varepsilon}}^2 \nonumber \\
        & \hspace{2cm} \leqslant \max_{d \in \{1,\dots, D\}} \lambda^{(d)} \big\| \widetilde{c} - c_\epsilon \big\|_{\R^{K_\varepsilon}}^2 \nonumber \\
        & \hspace{2cm} \leqslant \frac{\max_{d \in \{1,\dots, D\}} \lambda^{(d)}}{\sigma_{2D}^2} \, \Big\| A(0,T_\epsilon) (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2 \label{eq:inv_ineq} \\
        & \hspace{2cm} = \frac{\max_{d \in \{1,\dots, D\}} \lambda^{(d)}}{\sigma_{2D}^2} \bigg( \Big\| A(0,T_\epsilon)_1 (\widetilde{c} - c_\epsilon) \Big\|_{\R^D}^2 + \Big\| A(0,T_\epsilon)_2 (\widetilde{c} - c_\epsilon) \Big\|_{\R^D}^2 \bigg) \label{eq:mat_two_parts} \\
        & \hspace{2cm} = \frac{\max_{d \in \{1,\dots, D\}} \lambda^{(d)}}{\sigma_{2D}^2} \Big( \big\| y_{init} - \widetilde{y}_\epsilon(0) \big\|_{\R^D}^2 + \big\| y_{fin} - \widetilde{y}_\epsilon(T_\epsilon) \big\|_{\R^D}^2 \Big) \label{eq:recov_init_cond} \\
        & \hspace{2cm} \leqslant \frac{\max_{d \in \{1,\dots, D\}} \lambda^{(d)}}{\sigma_{2D}^2 \min_{d \in \{1,\dots, D\}} \lambda^{(d)}} \Big( \Big\| \Lambda^\frac{1}{2} \big (y_{init} - \widetilde{y}_\epsilon(0) \big) \Big\|_{\R^D}^2 + \Big\| \Lambda^\frac{1}{2} \big( y_{fin} - \widetilde{y}_\epsilon(T_\epsilon) \big) \Big\|_{\R^D}^2 \Big) \label{eq:equiv_norms} \\
        & \hspace{2cm} \leqslant \frac{\max_{d \in \{1,\dots, D\}} \lambda^{(d)}}{\sigma_{2D}^2 \min_{d \in \{1,\dots, D\}} \lambda^{(d)}} \, \delta \; ; \label{eq:constraints_hyp}
    \end{align}
    \begin{itemize}
        \item \eqref{eq:inv_ineq}: use the inequality
        \begin{equation*}
            \sigma_{2D}^2 \big\| \widetilde{c} - c_\epsilon \big\|_{\R^{K_\varepsilon}}^2 \leqslant \Big\| A(0,T_\epsilon) (\widetilde{c} - c_\epsilon) \Big\|_{\R^{2D}}^2
        \end{equation*}
        proved above and the fact that $\sigma_{2D} > 0$;
        \item \eqref{eq:mat_two_parts}: the matrices $A(0,T_\epsilon)_1, A(0,T_\epsilon)_2 \in \R^{D \times K_\varepsilon}$ are defined as follows:
        \begin{align*}
            & \bullet \quad A(0,T_\epsilon)_1 := \left(
            \begin{array}{ccccccc}
                \varphi_0(0) & \dots & \varphi_{K_{\varepsilon, 1}}(0) & & & & \\
                & & & \ddots & & & \\
                & & & & \varphi_0(0) & \dots & \varphi_{K_{\varepsilon, D}}(0)
            \end{array} \right) \; ; \\
            & \bullet \quad A(0,T_\epsilon)_2 := \left(
            \begin{array}{ccccccc}
                \varphi_0(T_\epsilon) & \dots & \varphi_{K_{\varepsilon, 1}}(T_\epsilon) & & & & \\
                & & & \ddots & & & \\
                & & & & \varphi_0(T_\epsilon) & \dots & \varphi_{K_{\varepsilon, D}}(T_\epsilon)
            \end{array} \right) \; ;
        \end{align*}
        in particular, they satisfy
        \begin{equation*}
            A(0,T_\epsilon) = \left(
            \begin{array}{c}
                A(0,T_\epsilon)_1 \\[2mm]
                A(0,T_\epsilon)_2
            \end{array} \right) \; ;
        \end{equation*}
        \item \eqref{eq:recov_init_cond}: by the definitions of the matrices $A(0,T_\epsilon)_1, A(0,T_\epsilon)_2$ and of the trajectory $\widetilde{y}_\epsilon = \Phi|_{\mathcal{Y}_\epsilon(0,T_\epsilon)}^{-1} c_\epsilon$, we have
        \begin{equation*}
            A(0,T_\epsilon)_1 \, c_\epsilon := \widetilde{y}_\epsilon(0) \qquad , \qquad A(0,T_\epsilon)_2 \, c_\epsilon := \widetilde{y}_\epsilon(T_\epsilon) \; ,
        \end{equation*}
        and by the fact that the vector $\widetilde{c}$ belongs to $\mathcal{B}(y_{init},y_{fin})$, we obtain
        \begin{equation*}
            A(0,T_\epsilon)_1 \, \widetilde{c} := y_{init} \qquad , \qquad A(0,T_\epsilon)_2 \, \widetilde{c} := y_{fin} \; ;
        \end{equation*}
        \item \eqref{eq:equiv_norms}: use the following inequality
        \begin{equation*}
            \forall x \in \R^D \qquad \min_{d \in \{1,\dots,D\}} \lambda^{(d)} \big\| x \big\|_{\R^D}^2 \leqslant \Big\| \Lambda^{\frac{1}{2}} x \Big\|_{\R^D}^2 \; ;
        \end{equation*}
        \item \eqref{eq:constraints_hyp}: use the hypothesis
        \begin{equation*}
            \Big\| \Lambda^\frac{1}{2} \big (\widetilde{y}_\epsilon(0) - y_{init} \big) \Big\|_{\R^D}^2 + \Big\| \Lambda^\frac{1}{2} \big (\widetilde{y}_\epsilon(T_\epsilon) - y_{fin} \big) \Big\|_{\R^D}^2 \leqslant \delta \; .
    \end{equation*}
    \end{itemize}
    By using once again \autoref{prop:phi_unitary} and by using the property that $c_0^\star$ is a minimiser, we obtain finally
    \begin{align*}
        \int_0^{T_\epsilon} \Big\| \Lambda^{\frac{1}{2}} \big( y_0^\star(t) - \widetilde{y}_\epsilon(t) \big) \Big\|_{\R^D}^2 \, dt 
            & = \Big\| \overline{\Lambda}^\frac{1}{2} (c_0^\star - c_\epsilon ) \Big\|_{\R^{K_\varepsilon}}^2 \\
            & \leqslant \Big\| \overline{\Lambda}^\frac{1}{2} (\widetilde{c} - c_\epsilon ) \Big\|_{\R^{K_\varepsilon}}^2 \\
            & \leqslant \frac{\max_{d \in \{1,\dots, D\}} \lambda^{(d)}}{\sigma_{2D}^2 \min_{d \in \{1,\dots, D\}} \lambda^{(d)}} \, \delta \; .
    \end{align*}
\end{proof}

\begin{lemma} \label{lem:continuity_pert}
    Let $A \in \R^{\widetilde{K} \times K}$ be a full rank matrix with $\widetilde{K} \leqslant K$ and let $b \in \R^{\widetilde{K}}$. Let $f, g :\R^K \longrightarrow \R$ be two $\mathcal{C}^2$-functions such that $f$ is strictly convex and such that the $C^2$-function $h_\eta := f + \eta \, g$ is strictly convex for all $\eta \in \mathcal{N}(0) \subseteq \R$, where $\mathcal{N}(0)$ is an open neighbourhood of $0$. We define the function $x^\star: \mathcal{N}(0) \longrightarrow \R^K$ as
    \begin{equation} \label{eq:opti_abst}
        x^\star(\eta) := \argmin_{Ax = b} h_\eta(x) \; ,
    \end{equation}
    which is well-defined. Then the function $x^\star$ is continuous at $0$.
\end{lemma}
\begin{proof}
    For all $\eta \in \mathcal{N}(0)$, the optimisation problem \eqref{eq:opti_abst} has a unique solution $x^\star(\eta) \in \R^K$ since the cost function is strictly convex and the constraint is affine. Further the cost function $h_\eta$ is a $\mathcal{C}^2$-function and the matrix $A$ is full rank by hypothesis. By Lagrange multiplier theorem \cite[p. 285]{F2000}, for all $\eta \in \mathcal{N}(0)$, there exists a unique vector $\lambda(\eta) \in \R^{\widetilde{K}}$ such that
    \begin{equation} \label{eq:lagrange}
        \nabla h_\eta \big( x^\star(\eta) \big) + A^T \lambda(\eta) = 0_{\R^K} \; .
    \end{equation}
    Define now $u : \R^K \times \mathcal{N}(0) \longrightarrow \R^K$ as follows
    \begin{equation*}
        u(x, \eta) = \nabla h_\eta \big( x \big) + A^T \lambda(\eta) \; .
    \end{equation*}
    Then, by equality \eqref{eq:lagrange}, we have
    \begin{equation*}
        u\big(x^\star(\eta), \eta \big) = 0_{R^K} \; ,
    \end{equation*}
    and the gradient $\nabla_x u$ of $u$ with respect to its first variable is equal to the Hessian matrix of $h_\eta$. Since $h_\eta$ is supposed to be strictly convex for all $\eta \in \mathcal{N}(0)$, its Hessian is positive definite and hence $\nabla_x u$ is invertible. By the implicit function theorem, we deduce the continuity of $x^\star$ at $0$.
\end{proof}

==> model_applications.tex <==
We now move to applying the above method to two different settings. 

\subsection{Fuel-efficient trajectories for aircraft} \label{subsec:appli_aero_model}

\todo{Notations for fuel flow and consumption ?}

In this subsection, we consider the aeronautic problem of reducing the total fuel consumption of an aircraft during the climb phase. This example illustrates the key role played by the reference trajectories since we are able to obtain very promising optimised trajectories thanks to a simple modelling involving few constraints; we refer to \cref{sec:appli_aero} for the numerical results. This motivates further studies on this problem using our methodology. For instance one could model environmental conditions or take into account Air Traffic Control constraints for more realistic modellings.

Here trajectories are supposed to be in a vertical plane and are defined by the altitude $h$, the Mach number $\M$ and the engines rotational speed $\N$ (expressed as a percentage of a maximal value). Hence a trajectory $y$ in this setting is a continuous $\R^3$-valued function defined on $[0,T]$, where $T$ is a maximal climb duration fixed by the user. Hence we have
\begin{equation*}
    \forall \, t \in [0,T] \qquad y(t) := \big( h(t), \M(t), \N(t) \big) \; .
\end{equation*}
The quantity to minimise is the total fuel consumption $\TFC: \mathcal{C}\big( [0,T], \R^3 \big) \longrightarrow \R_+$ which is defined via the fuel flow $\FF: \R^3 \longrightarrow \R_+$ as follows:
\begin{equation*}
    \TFC(y) := \int_0^T \FF\big(y(t)\big) \, dt \; .
\end{equation*}
\todo{footnote to refer to preceding notations}
Regarding the endpoints conditions, we require the trajectory to start at the altitude $h_0$ with Mach number $\M_0$ and to end at the altitude $h_T$ with Mach number $\M_T$. In particular, the reference trajectories we use have to verify these conditions.
% The average values of the starting and ending $\N$ computed using the reference flights are then used to set the endpoints conditions on the engines rotational speed.

\todo{itemize}
We consider also two additional constraints which are conventional in the aeronautic setting. The rate of climb, \emph{i.e.} the time-derivative of the altitude, has to be upper bounded by a given maximal value $\gamma_{max}$ during the whole climb and the Mach number should not exceed the maximum operational Mach ($\MMO$). We also consider a third constraint which permits to determine the duration of the climb: if we let denote $T^\star \in [0,T]$ the first time where the aircraft reaches $h_T$, then we require $\M(T^\star)$ to be equal to $\M_T$. Note that this constraint is satisfied by the reference trajectories.

Finally we mention that the fuel flow model $\FF$ is here estimated. To do so, we exploit the reference trajectories which contain recorded altitude, Mach number, engines power and fuel flow for each second of the flight. Having access to these data, we are in position to fit a statistical model. Here we consider a polynomial model of degree 2 to obtain at the end a quadratic program as explained in \cref{subsec:quad_model}. The prediction accuracy of the resulting estimated model is assessed in \cref{sec:appli_aero}.


\subsection{Maximising the work of a physical force along a path} \label{subsec:appli_phys_nautic}

Here we consider the following generic example: given a moving point in a force field, find a trajectory starting and ending at two different given points which maximises the work of the force along the trajectory while minimising the travelled distance. For instance, \todo{motion of point in wind -- nautic}. This second example demonstrates that our generic optimisation approach is flexible enough to take into account derivatives of trajectories and hence to cover dynamics settings.

To model this problem, we suppose without loss of generality that the trajectories are defined on the (time-)interval $[0,1]$ and we let  $V: \R^D \longrightarrow \R$ denote a vector field. Furthermore the trajectories are assumed here to be continuously differentiable, \emph{i.e.} they belong to $\mathcal{C}^1\big([0,1], \R^D \big)$. The work of $V$ along a trajectory $y \in \mathcal{C}^1\big( [0,1], \R^D \big)$ is defined as
\begin{equation*}
    W(y, \dot{y}) := \int_0^1 V\big(y(t)\big)^T \dot{y}(t) \, dt \; ;
\end{equation*}
here $\dot{y}$ denotes the derivative of $y$ with respect to the independent variable $t$. Moreover using Hamilton's principle in Lagrangian mechanics, it can be shown that the trajectory with constant velocity is the minimum of the following functional,
\begin{equation*}
    J(\dot{y}) = \int_0^1 \big\| \dot{y}(t) \big\|_2^2 \, dt \; ,
\end{equation*}
where the starting and ending points of $y$ are fixed and different. This functional can be then used to control the velocity of the moving point. It follows that minimising the cost function
\begin{equation*}
    F_\alpha(y, \dot{y}) := \alpha J(\dot{y}) - W(y, \dot{y}) = \int_0^1 \alpha \big\| \dot{y}(t) \big\|_2^2 - V\big(y(t)\big)^T \dot{y}(t) \, dt \; ,
\end{equation*}
where $\alpha \geqslant 0$ is arbitrarily chosen, is expected to lead to an optimised trajectory reflecting a trade-off between maximising the work and minimising the travelled distance. Further we require the trajectory to stay in the hypercube $[0,1]^D$ and to start and to end respectively at $y_0 \in [0,1]^D$ and $y_1 \in [0,1]^D$.

Now we remark that the above cost function involves the (time-)derivative $\dot{y}$. So one has to derive a formula permitting to compute the derivative of any trajectory $y = \Phi|_{\mathcal{Y}_\mathcal{K}}^{-1} c \in \mathcal{Y}_\mathcal{K}$ from its associated vector $c \in \R^K$, especially to compute the cost $\check{F}(c)$ (introduced in \cref{def:cost} and involved in the generic optimisation problem \eqref{eq:opt_proj_2}). For instance, this can be easily achieved by assuming that each element of the functional basis is continuously differentiable. Indeed we can differentiate in this case any $y \in \mathcal{Y}_\mathcal{K}$ as follows:
\begin{equation*}
    \forall \, d = 1, \dots, D \qquad \dot{y}^{(d)} =  \left( \frac{d}{dt} \Phi|_{\mathcal{Y}_\mathcal{K}}^{-1} c \right)^{(d)} = \sum_{k=1}^{K_d} c_k^{(d)} \dot{\varphi}_k \; .
\end{equation*}
We deduce then the following formula for $\check{F}(c)$ in the present setting:
\begin{equation*}
    \check{F}(c) := F_\alpha\left( \Phi|_{\mathcal{Y}_\mathcal{K}}^{-1} c, \frac{d}{dt} \Phi|_{\mathcal{Y}_\mathcal{K}}^{-1} c  \right) \; .
\end{equation*}
Here the vector $c$ contains information on both position and velocity, permitting especially to keep the problem dimension unchanged. To finish, let us remark that it is possible to make the above formula for $\check{F}(c)$ explicit with respect to $c$ for certain cost functions $F_\alpha$. For instance this is the case when $F_\alpha$ is quadratic leading to a quadratic function $\check{F}$.

